Symmetry resolved entanglement entropy of excited states in a CFT

We report a throughout analysis of the entanglement entropies related to different symmetry sectors in the low-lying primary excited states of a conformal field theory (CFT) with an internal U(1) symmetry. Our findings extend recent results for the ground state. We derive a general expression for the charged moments, i.e. the generalised cumulant generating function, which can be written in terms of correlation functions of the operator that define the state through the CFT operator-state correspondence. We provide explicit analytic computations for the compact boson CFT (aka Luttinger liquid) for the vertex and derivative excitations. The Fourier transform of the charged moments gives the desired symmetry resolved entropies. At the leading order, they satisfy entanglement equipartition, as in the ground state, but we find, within CFT, subleading terms that break it. Our analytical findings are checked against free fermions calculations on a lattice, finding excellent agreement. As a byproduct, we have exact results for the full counting statistics of the U(1) charge in the considered excited states.

==> sortbib <==
#!/ps/cdc/users/white/srw/bin/perl -w
# 1) Save this script into a file called sortbib.
# 2) Type chmod 755 sortbib.
# 3) Change the first line to identify the location of perl on your
#    machine. (Type "which perl" or "whereis perl".) 
# 4) Take a Latex file which uses \cite{} to reference \bibitem{}'s,
#    and type sortbib file.tex.

# Written by Steven R. White
# Usage: sortbib latexfile.tex
# Sort \bibitems in order by \cites
# Comments out unused bibitems, reports on citations without references,
# and makes a backup file file.tex.bak.
# sortbib understands Latex comments, and doesn't get fooled
# by \%, etc.

$\ = "\n";		# set output record separator

sub removecomments	# comments: %, \\%, \\\\%, etc
    {			# not comments: \%, \\\%, etc
    $_[0] =~ s/\\\\/\xbb\xbb/g;	# Change double \ to weird chars
    $_[0] =~ s/\\\%/\xcc\xcc/g;	# Change \% to weird chars
    $_[0] =~ s/\%[^\n]*\n//g;
    $_[0] =~ s/\xcc\xcc/\\\%/g; # Change back
    $_[0] =~ s/\xbb\xbb/\\\\/g;
    }

sub getcomments
    {
    local($txt) = @_;
    $txt =~ s/\\\\/\xbb\xbb/g;
    $txt =~ s/\\\%/\xcc\xcc/g;
    @bibco = ($txt =~ /(\%[^\n]*\n)/g);
    for($i=0; $i <= $#bibco; $i++)
	{
	$bibco[$i] =~ s/\xcc\xcc/\\\%/g;
	$bibco[$i] =~ s/\xbb\xbb/\\\\/g;
	}
    @bibco;
    }

foreach $file (@ARGV) 
    {
    `cp $file $file.bak`;
    open(FILE,"<$file");
    undef $/;
    $wholefile = <FILE>;
    close FILE;
    open(OUT,">sortbib.tmp");
    $dothebib = ($wholefile =~ /thebibliography/);
    $bibpat = '';
    if($dothebib)
	{
	$wholefile =~ /(\\begin\{thebibliography\}\{\d+\})/;
	$bibpat = $1;
	@fileparts = split( 
	/\\begin\{thebibliography\}\{\d+\}|\\end\{thebibliography\}/,
    				$wholefile,3);
	}
    else
	{
	$bibpat = "\\begin\{references\}";
	@fileparts = split( /\\begin\{references\}|\\end\{references\}/,
    				$wholefile,3);
	}
    $text = $fileparts[0];
    $text =~ s/\n+$/\n/;
    print OUT $text;
    &removecomments($text);
    $text =~ s/onlinecite/cite/g;

    @cites = ($text =~ /\\cite\{([^\}]*)\}/g);
    @citelist = split(/[\s\,]+/,join(",",@cites));
    @uniquecites = ();
    foreach $ci (@citelist)
	{
	push(@uniquecites,$ci) if !grep(/^$ci$/,@uniquecites);
	}
    $list = join("\n",@uniquecites);
    print "Citations:";
    print $list;
    print "";

    $references = $fileparts[1];
    @bibco = &getcomments($references);
    &removecomments($references);
    $references =~ s/\n\n/\n/g;
    @bibitems = split(/\\bibitem/,$references);
    %bibhash = ();
    @keyarray = ();
    for($i = 1; $i <= $#bibitems; $i++)
	{
	$bibitems[$i] =~ s/\n$//;
	$bibitems[$i] =~ /^\s*\{([^\}\s]+)\s*\}.*/;
	$key = $1;
	push(@keyarray,$key);
	$bibhash{$key} = $bibitems[$i];
	}
    print OUT "$bibpat";
    $, = '';		# set output field separator
    foreach $key (@uniquecites)
	{
	if(exists $bibhash{$key})
	    { print OUT "\\bibitem",$bibhash{"$key"},"\n"; }
	else
	    { print "No bibitem for ", $key; }
	delete $bibhash{$key};
	}
    print OUT join("\n",@bibco) if ($#bibco != 0);
    print OUT "\\end\{references\}\n" if !$dothebib;
    print OUT "\\end\{thebibliography\}\n" if $dothebib;
    $first = 1;
    while(($key,$value) = each %bibhash)
	{
	$value =~ s/\n/\n\%/g;
	print OUT "\n\%Unused bibitems\n" if $first == 1;
	print "\n\%Unused bibitems\n" if $first == 1;
	$first = 0;
	print OUT "\%","\\bibitem",$value;
	print "\%","\\bibitem",$value;
	}
    $lastpart = $fileparts[2];
    $lastpart =~ s/\n$//;
    $lastpart =~ s/^\n+//;
    print OUT $lastpart;
    close OUT;
    `mv sortbib.tmp $file`;
    }


